Semantically Constrained Memory Allocation (SCMA) for Embedding in Efficient Recommendation Systems

Deep learning-based models are utilized to achieve state-of-the-art performance for recommendation systems. A key challenge for these models is to work with millions of categorical classes or tokens. The standard approach is to learn end-to-end, dense latent representations or embeddings for each token. The resulting embeddings require large amounts of memory that blow up with the number of tokens. Training and inference with these models create storage, and memory bandwidth bottlenecks leading to significant computing and energy consumption when deployed in practice. To this end, we present the problem of \textit{Memory Allocation} under budget for embeddings and propose a novel formulation of memory shared embedding, where memory is shared in proportion to the overlap in semantic information. Our formulation admits a practical and efficient randomized solution with Locality sensitive hashing based Memory Allocation (LMA). We demonstrate a significant reduction in the memory footprint while maintaining performance. In particular, our LMA embeddings achieve the same performance compared to standard embeddings with a 16$\times$ reduction in memory footprint. Moreover, LMA achieves an average improvement of over 0.003 AUC across different memory regimes than standard DLRM models on Criteo and Avazu datasets

==> approach.tex <==
%\newpage

\section{Proposal}
\subsection{SSM Embeddings}
Consider a large weight matrix W to be learned as a part of an end-to-end learning algorithm. If W has no particular relative structure, such as a weight matrix of a MLP layer, the best we can do under a given memory $\mathcal{M}$ and memory budget $m=|\mathcal{M}|$ is to share weight randomly \cite{hashtrick}. However, if $\mathcal{M}$ is allocated to a special weight matrix, embedding tables $\mathbf{E}$, which store embedding for different values $v$ in a categorical variable $V$, we can exploit the potential structure contained in the semantic information w.r.t the categorical values. The relation among the values can be captured by the similarities among the embeddings. High similarity among multiple values indicate redundancy of weights in $\mathbf{E}$. This situation implies that embedding for a value can be inferred from other highly similar values and therefore does not need to be stored explicitly.


%Consider a piece of memory $\mathcal{M}$ you aim to learn as a part of an end-to-end learning system. If $\mathcal{M}$ is arbitrary and has no structure that you can exploit, the best you can do under budget is use the hashing trick on the lines of \cite{hashtrick} to share weights. But, the situation is different when $\mathcal{M}$ is a special piece of memory like embedding table $\mathbf{E}$. Embeddings are supposed to store semantic information about the categorical values. These values share some relationship with each other that is captured via similarity between their embeddings. High similarity among multiple values indicate redundancy in the data stored in $\mathbf{E}$. Essentially this means that embedding for a value can be inferred from other highly similar values and need not be stored explicitly. In SSM Embeddings, we put to use this semantic structure. Assume for now, we know the similarity structure of values say $\mathcal{S}$. We force the embeddings of the values $v_1,v_2$ with similarity $\mathcal{S}_{v_1 v_2}$ to consistently share $\mathcal{S}_{v_1 v_2}$ fraction of memory locations where consistent sharing is defined as follows

%Consider the memory $\mathcal{M}$ under given memory budget, containing the values (i.e. weights) to be updated (i.e., learned) as part of an end-to-end learning algorithm. If $\mathcal{M}$ has no particular relative structure, such as weights arbitrarily arranged in a matrix, then to satisfy the memory budget, we can utilize well know techniques \cite{hashtrick} to randomly share the weights. However, if $\mathcal{M}$ is allocated to embedding tables $\mathbf{E}$ for categorical variables with values $v$ represented as embeddings $e \in \mathbf{E}$, then we can exploit potential structure contained in the semantic information with respect to categorical values. The relation among the values can be captured by the similarities among the embeddings. High similarity among multiple values indicate redundancy of weights in $\mathbf{E}$. This situation implies that embedding for a value can be inferred from other highly similar values and therefore does not need to be stored explicitly.

SSM embeddings take advantage of semantic structure among the categorical variables to reduce the memory burden and increase efficiency of learning. Given the similarity structure of values $\mathbb{S}$, we constrain embedding of values $v_i$ and $v_j$ with similarity $\mathbb{S}_{v_i v_j}$ to {\em consistently share} $\mathbb{S}_{v_i v_j}$ fraction of memory locations where consistent sharing is defined as follows.

\begin{defn}[Consistent Sharing]
Two embeddings $e_1$, $e_2 \in \mathbb{R}^d$ are said to consistently share a memory location $x \in \mathcal{M}$, if there exists $i \in \{0,1,\ldots,d{-}1\}$ such that $e_1[i]$ and $e_2[i]$ are essentially same memory location $x$ and hence share the value at $x$.
\end{defn}

\begin{figure}[h]
    \centering
    \includegraphics[trim = 10 0 0 0, clip,scale=0.6]{figures/hashing-diagram-2.pdf}
    \caption{The embeddings $e_{v_1}$ and $e_{v_2}$ retrieved from $\mathcal{M}_{\mathbb{S}_J}$ consistently share two memory locations as the minwise functions $l_1$ and $l_3$ collide for $D_{v_1}$ and $D_{v_2}$.}
    \label{fig:my_label}
\end{figure}
%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.4]{figures/SSME.png}
%    \caption{The embeddings $e_{v_1}$ and $e_{v_2}$ retrieved from $\mathcal{M}_{J}$ consistently share two memory locations as the minwise functions $l_1$ and $l_3$ collide for $\mathcal{D}_{v_1}$ and $\mathcal{D}_{v_2}$ }
%    \label{fig:my_label}
%\end{figure}

%\begin{defn}[Consistent Sharing]
%Two embeddings $e_1$ and $e_2$ of dimension d are said to consistently share a memory location x, if there is a $i \in \{0,1,\ldots,d-1\}$ such that $e_1[i]$ and $e_2[i]$ are essentially same memory location x and hence share the value at x
%\end{defn}
We prove in section \ref{sec:theory}, that under some assumptions, sharing memory indeed results in similarity. SSM Embeddings learn this piece of memory while retrieving embeddings constrained by $\mathbb{S}$. We will denote by $\mathcal{M}_{\mathbb{S}}$ the memory $\mathcal{M}$ that is used to retrieve SSM embeddings with similarity constraint $\mathbb{S}$. There are still two issues that we need to resolve 1) $\mathbb{S}$ is not known a priori. 2) We need a way to impose this $\mathbb{S}$ and retrieve $\mathbf{E}$ from $\mathcal{M}_\mathbb{S}$.

Firstly, if we represent each value by the set of ids of samples in which it occurs in data, we can find a similarity structure imposed by Jaccard Similarity ($J$). Let $\mathcal{D}_v$ denote the set of such indices from data $\mathcal{D}$ for value $v$ and the similarity structure thus obtained be $\mathbb{S}_J$. We conjecture that $\mathbb{S}_J$ is a good proxy for $\mathcal{S}$. \verify{Also, we empirically confirm that this is the case in Criteo. If true add plot}. We will denote $\mathcal{M}_\mathbb{S}$ by $\mathcal{M}_J$ while using similarity structure $\mathbb{S}_J$. Secondly, we use locality sensitive minwise hash functions using these sets to approximately impose the memory sharing commensurate to Jaccard similarity. The probability of collision of a min-wise hashing applied to sets $D_{v_1}$ and $D_{v_2}$ is equal to the $J(D_{v_1}, D_{v_2})$
\begin{equation}
    P_{l\in\mathcal{L}}(l(D_{v_1}) == l(D_{v_2})) = J(D_{v_1}, D_{v_2})
\end{equation}
So in expectation, $v_1$ and $v_2$ consistently share $J(D_{v_1}, D_{v_2})$ fraction of memory locations. Same mapping is used to retrieve the embeddings from $\mathcal{M}_J$. Formally, given a value v, its embedding $e_v \in R^d $ is retrieved from constrained memory  $\mathcal{M}_J$ by using d independent minwise hash functions $\{ l_i \}_{i=1}^d$ in the following manner
\begin{equation*}
    e_v[i] = \mathcal{M}_J [l_i(\mathcal{D}_v)]
\end{equation*}
To retrieve an embedding every time, we would need to store $\mathcal{D}$. This would seem like a problem as $\mathcal{D}$ can potentially be very large. However, under the i.i.d assumption of the each sample in $\mathcal{D}$,  we only need a small sub-sample of $\mathcal{D}$, to accurately estimate the true Jaccard similarity on $\mathcal{D}$. Hence, the size of actual data required, say $\mathcal{R}$(for representation of values), is very small as compared to the embedding table. We also theoretically prove this in the section \ref{sec:theory}.


\input{theory}
\section{SSM Embeddings in Recommendation Models}
We use SSM Embeddings in recommendation model by having all the embedding tables simulated from a single piece of similarity constrained memory $\mathcal{M}_{J}$. We use Jaccard similarity from the data $\mathcal{D}$. The scheme is shown in figure \ref{fig:ssmdlrm}

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/ssme_dlrm_n.png}
    \caption{SSM Embeddings in DLRM mdoel}
    \label{fig:ssmdlrm}
\end{figure}
\textbf{Forward Pass:}
The forward pass requires us to find embeddings of size, say d, for a set of values, $V_{batch}$, present in the batch. In naive embeddings, this is achieved by a simple indexing operation. In SSM embeddings, we first collect $\{D_v  | v \in V_{batch} \}$ and then apply minwise hashing with d hash functions to give us a matrix of indices $ID \in R^{|V| \times d}$. We use this matrix to index into memory $\mathcal{M}_J$
\begin{equation}
    E_{batch} = \mathcal{M}_J[ID]
\end{equation}
\textbf{Backward Pass:}
The memory $\mathcal{M}_J$ contains the parameters which are used to construct embeddings. Hence, in backward pass, the gradient of parameters in $\mathcal{M}_{J}$ is computed and the parameters are updated. The exact functional dependence of result on a parameter in $\mathcal{M}_J$ is complex as it is implemented via lsh mappings. Auto gradient computation packages of deep learning libraries like pytorch and tensorflow are used for the gradient computation.

\textbf{Memory Comparison}
\begin{table}[]
\centering
\begin{tabular}{@{}|l|l|@{}}
\toprule
Original Embedding     & $ \mathbb{O}(|S| \times d) $              \\ \midrule
SSM Embedding & $ \mathbb{O}(m + kd + |D'| )$ \\ \bottomrule
\end{tabular}
\caption{Memory Complexity}
\label{tab:mem}
\end{table}
Suppose the combined set of all values of all categorical features is S. Let the dimension of the embedding be d. Then the size of the memory used by naive embeddings is $\mathbb{O}(|S|d)$. The linear dependence on d and very large typical size of set S makes it difficult to train and deploy large dimensional embedding models. SSM Embedding memory on the other hand does not depend directly on $|S|$ . The memory cost of SSM comprises of (1.) constrained memory used : $m=|\mathcal{M_{J}}|$ (2.) Size of sub sample of data used. (3.) cost of storing lsh function parameters. The effect of m on similarity and shared memory is captured in theorem 1 and 2. The effect of number of samples is shown in theorem 3. Generally the number of non-zeros stored is way smaller than $(|S|d)$. For example in criteo, sub sample we used had less than 3M integers as compared to 50-540M parameters of the models we train. The space complexity to store d lsh hash functions is $\mathbb{O}(kd)$ where k depends on universality of hash function we use to mimic permutation in lsh function and d is dimension of the embedding. Again, this is very small as compared to $|S|d$. This is summarized in table \ref{tab:mem}. 

\input{plot_mainres_wide} % required in experiments. added here for positioning
\textbf{Handling very sparse features} For very sparse features, the embedding quality does not really affect the accuracy of the model \cite{MDTrick19}. Also, it is diffcult to get good estimate of jaccard similarity for this using a small subsample. Due to both these reasons, for very sparse features, we randomly map each element of its embedding into the $\mathcal{M}_J$. Essentially we revert to hashing trick for such values.


% things to talk about
% diagram
% single memory shared across the different embedding tables
% Embedding from $\mathcal{M_{J}}$
% Memory Comparison
% forward pass. getting embedding at each training step.
% backward pass. updating weights. 
% 

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.3]{figures/hashingtrick.png}
%    \caption{Hashing Trick: Embeddings obtained from hashing trick using mappings drawn from universal hash families}
%    \label{fig:hashtrick}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.3]{figures/ssmembedding.png}
%    \caption{SSM Embedding: Embeddings obtained from using LSH mapping }
%    \label{fig:my_label}
%\end{figure}

==> hyperparam_exp_table.tex <==
\begin{table}[]
    \centering
    % \setlength{\belowdisplayskip}{-0.cm}
    \begin{tabular}{|c V{3} c|c|c|c|}
        \hline
        Variable & 
        $n_h$ & 
        $\alpha$ & 
        $n_s$ &
        \tabincell{c}{number of \\parameters}\\
        \hline
        $n_h$ &
        \tabincell{c}{-}&
        %\tabincell{c}{1,2,\\4,8} &
        32x &
        125k &
        \~36M \\ 
        \hline
        $\alpha$& 
        \tabincell{c}{2}&
        \tabincell{c}{-}&
        %\tabincell{c}{32x,16x,\\8x,4x,2x}&
        \tabincell{c}{125k} &
        \~270M
        \\
        \hline
        $n_s$& 
        \tabincell{c}{2}&
        \tabincell{c}{32x}&
        \tabincell{c}{-}&
        %\tabincell{c}{10k,75k,\\125k,\\250k,500k} &
        \~36M\\
        \hline
    \end{tabular}
    \caption{Hyperparameter experiments setup}
    % \setlength\belowdisplayskip{-10pt} 
    \label{tab:hyperparameter_experiments_setup}
    \vspace{-10pt} 
\end{table}

==> plot_mainres.tex <==
\begin{figure}\label{fig:main_experiment}
\begin{subfigure}{.49\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{figures/criteo/Criteo_AUC.png}
    \caption{Criteo - AUC}
    \label{fig:criteo_auc}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{figures/avazu/Avazu_AUC.png}
    \caption{Avazu - AUC}
    \label{fig:avazu_auc}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{figures/criteo/Criteo_accuracy.png}
    \caption{Criteo - Accuracy}
    \label{fig:criteo_accuracy}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{figures/avazu/Avazu_accuracy.png}
    \caption{Avazu - Accuracy}
    \label{fig:avazu_accuracy}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{figures/criteo/Criteo_loss.png}
    \caption{Criteo - Loss}
    \label{fig:criteo_loss}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{figures/avazu/Avazu_loss.png}
    \caption{Avazu - Loss}
    \label{fig:avazu_loss}
\end{subfigure}
\caption{AUC, Accuracy, and Loss against memory regimes (number of parameters) on Criteo and Avazu}
\label{fig:main_experiment}
\vspace{-0.5cm}
\end{figure}

==> theory.tex <==
\subsection{Analysing SSM Embeddings}\label{sec:theory}

Proofs of all the theorems are provided in the supplemental.

%\begin{thm}\label{thm:thm_1}
%Given embeddings $e_{v_i}, e_{v_j} \in \mathbb{R}^d$ corresponding to categorical values $v_i$, $v_j$ and dataset $D_{v_i}$, $D_{v_j}$. Define the Jaccard similarity as $J{=}J(D_{v_i}, D_{v_j})$. Let $|\mathcal{M}_{\mathbb{S}_J}|{=}m{>}0$ and $0{<}f{<}1$ be the fraction of consistently shared memory between $e_{v_i}$ and $e_{v_j}$ under $\mathcal{M}_{\mathbb{S}_J}$. Then, the distribution on the $J$ when retrieved from $\mathcal{M}_{\mathbb{S}_J}$ is parameterized by expectation and variance as
%\begin{align*}
%&\mathbb{E}(f) = J + \frac{(1{-}J)}{m} \quad , \quad
%Var(f) = \frac{\mathbb{E}(f) (1{-}\mathbb{E}(f))}{d},\\
%& \text{respectively. Then, for any $\delta>0$, we have}\\
%& \mathrm{Pr}\left(|f{-}J| > \delta \mathbb{E}(f) + \frac{(1{-}J)}{m}\right) %\leq 2 \exp\left\{\frac{-d \mathbb{E}(f) \delta^2}{3}\right\}.    
%\end{align*}
%\end{thm}



\begin{thm}[SSM retrieval implies shared memory] \label{thm:thm_1}
For two distinct values $v_1$ and $v_2$, let the corresponding datasets be $D_{v_1} and D_{v_2}$, jaccard similarity be $J = J(D_{v_1}, D_{v_2}$, SSM retreived embeddings be $e_{v_1}$ and $e_{v_2}$. Let $|\mathcal{M}_J| = m > 0$. The fraction of consistently shared memory, $0 \leq \hat{f} \leq 1$, between $e_{v_1}$ and $e_{v_2}$ when $e_{v_1}$ and $e_{v_2}$ are retrieved from $\mathcal{M}_J$ is distributed as follows.

\begin{align*}
&\mathbb{E}(f) = J + \frac{(1{-}J)}{m} \quad , \quad
Var(f) = \frac{\mathbb{E}(f) (1{-}\mathbb{E}(f))}{d},\\
& \text{respectively. Then, for any $\delta>0$, we have}\\
& \mathrm{Pr}\left(|f{-}J| > \delta \mathbb{E}(f) + \frac{(1{-}J)}{m}\right) \leq 2 \exp\left\{\frac{-d \mathbb{E}(f) \delta^2}{3}\right\}.    
\end{align*}
\end{thm}

\textbf{Interpretation:} According to Theorem \ref{thm:thm_1}, SSM procedure implies that consistently shared fraction $f$ between two embeddings is closely related to their Jaccard similarity $J$. The expected value of $f$ is not exactly $J$ since the minhash value generated has to be rehashed into $\mathcal{M}_{J}$, which leads to random collisions. However, even a small memory size of 10\textsc{mb} would have $m{>}10^6$. Therefore, for all practical cases, $\mathbb{E}(f)$ is $J$. Chernoff concentration inequality gives strong bound on deviation of $f$ from $J$. The $95\%$ confidence intervals for $f$ against $J$ is shown in Figure \ref{fig:err} for various values of $d$.


%\begin{thm}\label{thm:thm_2}
%Given embeddings $e_{v_i}, e_{v_j} \in \mathbb{R}^d$ corresponding to categorical values $v_i$, $v_j$ and dataset $D_{v_i}$, $D_{v_j}$. Define the Jaccard similarity as $J{=}J(D_{v_i}, D_{v_j})$ and cosine similarity as $\cos(e_{v_i},e_{v_j})$. Let $|\mathcal{M}_{\mathbb{S}_J}|{=}m{>}0$ be initialized such that $\mathcal{M}_{\mathbb{S}_J}[k] \sim Bernoulli(1/2,\{-1,+1\})$ independently for $k=0,1,\ldots,m{-}1$. Then, the distribution on $J$ and $\cos(e_{v_i},e_{v_j})$  when retrieved from $\mathcal{M}_{\mathbb{S}_J}$ is parameterized by expectation
%\begin{equation*}
%\mathbb{E}(\cos(e_{v_i},e_{v_j})) = J + \frac{(1{-}J)}{m}.
%\end{equation*}
%Let $\Gamma = \mathbb{E}(\cos(e_{v_i},e_{v_j}))$, we have variance as
%\begin{equation*}
%Var(\cos(e_{v_i},e_{v_j})) = \frac{1-\Gamma^2}{d} + \frac{2(1-\Gamma)(d-1)}{dm^2}.
%\end{equation*}
%Then, for any $\delta>0$, we have
%\begin{equation*}
%\mathrm{Pr}\left( |\cos(e_{v_i},e_{v_j})-J| \geq \delta\Gamma + %\frac{(1-J)}{m}\right) \leq \frac{(1-\Gamma^2)}{d\delta^2\Gamma^2}.
%\end{equation*}
%\end{thm}


\begin{thm}[SSM retrieval implies similarity]\label{thm:thm_2}
For two distinct values $v_1$ and $v_2$, let the corresponding datasets be $D_{v_1} and D_{v_2}$ , jaccard similarity be $J = J(D_{v_1}, D_{v_2}$ and SSM retreived embeddings be $e_{v_1}$ and $e_{v_2}$. Let $\mathcal{M_J}$, $|\mathcal{M_J}|=m$ be initialized as $\mathcal{M}_J[i] \sim \textrm{Bernoulli}(1/2, \{-1,+1\})$ independently for $i=0,1,\ldots,m-1$. Then the cosine similarity between $e_{v_1}$ and $e_{v_2}$, i.e $cosine(e_{v_1},e_{v_2}$), denoted by $\hat{C}_s$, is distributed as 
\begin{equation*}
\mathbb{E}(\hat{C}_s) = J + \frac{(1{-}J)}{m}.
\end{equation*}
\begin{equation*}
Var(\hat{C}_s) = \frac{1-\mathbb{E}(\hat{C}_s)^2}{d} + \frac{2(1-\mathbb{E}(\hat{C}_s))(d-1)}{dm^2}.
\end{equation*}
Then, for any $\delta>0$, we have
\begin{equation*}
\mathrm{Pr}\left( |\hat{C}_s-J| \geq \delta \mathbb{E}(\hat{C}_s) + \frac{(1-J)}{m}\right) \leq \frac{(1-\mathbb{E}(\hat{C}_s)^2)}{d\delta^2\mathbb{E}(\hat{C}_s)^2}.
\end{equation*}
\end{thm}
 \textbf{Interpretation:} 
Theorem \ref{thm:thm_2} suggests that the cosine similarity between embeddings are closely distributed around their Jaccard similarity $J$. We prove this result under a specific distribution of values in $\mathcal{M}_{J}$ for simplicity. General analysis of learned memory would be impossible. We cannot use Chernoff inequality since there is added complexity in this random variable (see Supplemental). Therefore, we use Chebysev's concentration inequality which gives us a looser bound. Again, in any reasonable system, $m$ is sufficiently large. Thus, if we ignore $1/m$, then expected cosine similarity essentially equal to $J$. The probable region for cosine similarity under various values of $J$ and $d$ is shown in Figure \ref{fig:err}. For large $m$, these shaded regions are nearly the 95\% confidence interval for cosine similarity.

       \begin{figure}
\begin{subfigure}{.48\linewidth}
  \centering
  \includegraphics[width=.98\linewidth]{figures/theorem_plots/thm1.png}
  \caption{Probable region for shared memory fraction vs J }
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.48\linewidth}
  \centering
  \includegraphics[width=.98\linewidth]{figures/theorem_plots/thm2.png}
  \caption{Probable region for cosine similarity vs J}
  \label{fig:sf2}
\end{subfigure}
\caption{$\mu \mp 1.96 \sigma $ regions for different values of $d$ as per theorems 1 and 2. For $\hat{f}$ this is 95\% confidence intervals }
\label{fig:err}
\end{figure}
\begin{thm}[Sample of Data required is small] \label{thm:thm_3}
Assuming a uniform sparsity of each value, s, the Jaccard Similarity of two values x and y,say $J=J(D_x, D_y)$ when estimated from a i.i.d subsample $D' \subseteq \mathcal{D}$, $|D'| = n$ is distributed around J as follows.
\begin{equation}
    | \mathbb{E}(\hat{J}) - J | \leq \epsilon J
\end{equation}
\begin{equation}
    |\mathbb{V}(\hat{J}) - A| \leq 2\epsilon(A+2J^2)
\end{equation}
where $A =\frac{J}{2ns} (1+J -2sJ)$ with probability $(1-\delta)$ where $\delta = \frac{1+J - 2s}{2ns\epsilon^2} $
\end{thm}

\textbf{Interpretation:} The bound given by this theorem is loose due to the approximations done to analyse this random variable. Appendix A shows the exact analysis. Nonetheless, it can be seen that for a given value of $\delta$, we can control $\epsilon$ and $A$ by controlling $ns$ which is the number of non-zeros per value. As ns increases, both the variance and deviation of expected value from J decreases rapidly. In practice, section \ref{sec:datapoints} shows we only need around 100K samples for criteo dataset out of 4.5M samples.

